Correlated Random Matrices: Band Rigidity and Edge Universality

We prove edge universality for a general class of correlated real symmetric or complex Hermitian Wigner matrices with arbitrary expectation. Our theorem also applies to internal edges of the self-consistent density of states. In particular, we establish a strong form of band rigidity which excludes mismatches between location and label of eigenvalues close to internal edges in these general models.

==> packages_and_notation_shape.tex <==
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc} 
\usepackage[p,osf]{cochineal}
\usepackage[scale=.95,type1]{cabin}
\usepackage[zerostyle=c,scaled=.94]{newtxtt}
\usepackage{graphicx} 
\newlength\figureheight 
\newlength\figurewidth 
\usepackage{color,bm}
\usepackage{amsmath,amssymb,amsthm,mathrsfs,amsfonts,dsfont,braket} 
\usepackage[foot]{amsaddr}
\usepackage{enumerate,titlesec} 
\usepackage{booktabs,changepage}
\usepackage{xspace,afterpage,tocvsec2} 
\usepackage[printonlyused,withpage]{acronym} 
\usepackage{rotating} 
\usepackage{ltablex}
\usepackage{dsfont,xstring}
\RequirePackage{setspace}
\usepackage{makecell}
\usepackage{mathrsfs} 
\usepackage[pdfencoding=auto,psdextra]{hyperref}
\usepackage[dvipsnames]{xcolor}
\usepackage[ocgcolorlinks]{ocgx2}
\hypersetup{breaklinks,colorlinks=true,linkcolor=MidnightBlue,citecolor=MidnightBlue,urlcolor=MidnightBlue}
\usepackage{etoolbox}
%\usepackage{microtype} 
\usepackage{grffile}
\usepackage{subcaption}
\renewcommand\thesubfigure{\textsc{\alph{subfigure}}}
\usepackage{csquotes}
%\usepackage{refcheck} 
%\lineskiplimit=-100pt\relax
\DeclareMathSizes{10.95}{10}{7}{5}
\setlength{\textwidth}{\paperwidth}
\setlength{\textheight}{\paperheight}
\addtolength{\textwidth}{-3.5cm}
\addtolength{\textheight}{-3.5cm}
\addtolength{\footskip}{\baselineskip}
\calclayout

\usepackage[style=phys,url=false,doi=false,isbn=false,eprint=true,datamodel=mrnumber,sorting=nty,maxbibnames=99,backref=false,block=space,backend=biber]{biblatex}
\renewbibmacro{in:}{}
\DefineBibliographyStrings{english}{%
  backrefpage = {$\hookrightarrow$~},% originally "cited on page"
  backrefpages = {$\hookrightarrow$~},% originally "cited on pages"
}
\bibliography{references}
\renewcommand*{\bibfont}{\scriptsize}
\DeclareFieldFormat[article]{title}{\emph{#1}} 
\DeclareFieldFormat{mrnumber}{%
  \ifhyperref
    {\href{http://www.ams.org/mathscinet-getitem?mr=#1}{\nolinkurl{MR#1}}}
    {\nolinkurl{#1}}}
\renewbibmacro*{doi+eprint+url}{%
  \iftoggle{bbx:doi}
    {\printfield{doi}}
    {}%
  \newunit\newblock
  \printfield{mrnumber}%
  \newunit\newblock
  \iftoggle{bbx:eprint}
    {\usebibmacro{eprint}}
    {}%
  \newunit\newblock
  \iftoggle{bbx:url}
    {\usebibmacro{url+urldate}}
    {}}

\patchcmd{\abstract}{\scshape\abstractname}{\textbf{\abstractname}}{}{}
\makeatletter
\titlespacing*{\subsubsection}{2.5ex}{0.5ex}{1ex}
\makeatletter
\renewcommand\subsection{\@startsection{subsection}{2}%
  \z@{.5\linespacing\@plus.7\linespacing}{-.5em}%
  {\normalfont\bfseries}}
\makeatother

\makeatletter
\def\section{\@startsection{section}{1}%
\z@{.7\linespacing\@plus\linespacing}{.5\linespacing}%
{\normalfont\bfseries\centering}}
\makeatother

\makeatletter
%Table of Contents
\setcounter{tocdepth}{3}

% Add bold to \section titles in ToC and remove . after numbers
\renewcommand{\tocsection}[3]{%
  \indentlabel{\@ifnotempty{#2}{\bfseries\ignorespaces#1 #2\quad}}\bfseries#3}
% Remove . after numbers in \subsection
\renewcommand{\tocsubsection}[3]{%
  \indentlabel{\@ifnotempty{#2}{\ignorespaces#1 #2\quad}}#3}
%\let\tocsubsubsection\tocsubsection% Update for \subsubsection
%...
\newcommand\@dotsep{4.5}
\def\@tocline#1#2#3#4#5#6#7{\relax
  \ifnum #1>\c@tocdepth % then omit
  \else
    \par \addpenalty\@secpenalty\addvspace{#2}%
    \begingroup \hyphenpenalty\@M
    \@ifempty{#4}{%
      \@tempdima\csname r@tocindent\number#1\endcsname\relax
    }{%
      \@tempdima#4\relax
    }%
    \parindent\z@ \leftskip#3\relax \advance\leftskip\@tempdima\relax
    \rightskip\@pnumwidth plus1em \parfillskip-\@pnumwidth
    #5\leavevmode\hskip-\@tempdima{#6}\nobreak
    \leaders\hbox{$\m@th\mkern \@dotsep mu\hbox{}\mkern \@dotsep mu$}\hfill
    \nobreak
    \hbox to\@pnumwidth{\@tocpagenum{\ifnum#1=1\bfseries\fi#7}}\par% <-- \bfseries for \section page
    \nobreak
    \endgroup
  \fi}
\AtBeginDocument{%
\expandafter\renewcommand\csname r@tocindent0\endcsname{0pt}
}
\def\l@subsection{\@tocline{2}{0pt}{2.5pc}{5pc}{}}
\makeatother

\newtheorem{theorem}{Theorem}
\numberwithin{theorem}{section}
\numberwithin{equation}{section}
\newtheorem{assumption}{Assumption}
\renewcommand*{\theassumption}{(\Alph{assumption})}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{fact}{Fact}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem*{genericthm*}{Assumption \ref{assumption correlations}'}
\newtheorem*{assCD}{Assumption (CD)}

\newcommand{\av}{\mathrm{av}}
\newcommand{\GUE}{\mathrm{GUE}}
\newcommand{\GOE}{\mathrm{GOE}}
\newcommand{\cusp}{\mathrm{cusp}}
\newcommand{\hs}{\mathrm{hs}}
\newcommand{\ii}{\mathrm{i}}
\renewcommand*{\acffont}[1]{{\normalsize\itshape #1}}
\renewcommand*{\acfsfont}[1]{{\normalsize\upshape #1}} 
\newcommand{\inD}[1]{\quad\text{in}\quad\DD_{#1}^\delta}
\newcommand{\inG}[1]{\quad\text{in}\quad\GG_{#1}^\delta}
\newcommand{\As}{\mathcal{A}}
\newcommand{\1}{\mathds{1}}
\newcommand{\R}{\mathbb{R}}  % The real numbers.
\ifdefined\C\renewcommand{\C}{\mathbb{C}}\else\newcommand{\C}{\mathbb{C}}\fi % Complex numbers
\newcommand{\N}{\mathbb{N}}  % Positive integers. 
\newcommand{\cM}{\mathcal{M}}  % Positive integers. 
\newcommand{\cE}{\mathcal{E}}  % Positive integers. 
\newcommand{\cF}{\mathcal{F}}  % Positive integers. 
\newcommand{\cu}{\mathfrak{c}}
\newcommand{\bu}{\mathfrak{b}}
\newcommand{\init}{\mathrm{in}}
\newcommand{\ed}{\mathfrak{e}}
\newcommand{\mi}{\mathfrak{m}}
\newcommand{\cG}{\mathcal{G}}  % Positive integers. 
\newcommand{\Hi}{\mathcal{H}}  % Hilbert space
\newcommand{\HC}{\mathbb{H}}  % Hilbert space
\newcommand{\BV}{BV}  %BV
\newcommand{\wt}{\widetilde}  %BV
\newcommand{\wh}{\widehat} 
\newcommand{\fc}{\text{fc}}
\newcommand*{\equal}{=}
\newcommand{\deq}{%
  \mathrel{\vbox{\offinterlineskip\ialign{%
    \hfil##\hfil\cr
    $\scriptscriptstyle d$\cr
    \noalign{\kern.1ex}
    $=$\cr
}}}}
\renewcommand{\star}{$^*$}
\newcommand{\Z}{\mathbb{Z}}  % Integers
\newcommand{\DD}{\mathbb{D}}  % Integers
\newcommand{\GG}{\mathbb{G}}  % Integers
\newcommand{\CC}{\mathcal{C}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\vz}{\mathbf{z}}
\newcommand{\Tuple}[1]{
\left(\,
\StrSubstitute{#1}{|}{\;\middle\vert\;}[\temp]%
\temp
\,\right)
}
\newcommand{\tuple}[1]{
(\,
\StrSubstitute{#1}{|}{\;\vert\;}[\temp]%
\temp
\,)
}
\newcommand{\vw}{\mathbf w}
\newcommand{\NN}{\mathcal{N}}
\newcommand{\vu}{\mathbf u}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vb}{\mathbf b}
\newcommand{\vl}{\mathbf l}
\newcommand{\vm}{\mathbf m}
\newcommand{\va}{\mathbf a}
\newcommand{\vp}{\mathbf p}
\newcommand{\vf}{\mathbf f}
\newcommand{\vd}{\mathbf d}
\renewcommand{\SS}{\mathcal{S}}
\newcommand{\Q}{\mathbb{Q}}  % Rational numbers. 
\newcommand{\K}{\mathbb{K}} % Number field
\newcommand{\LO}{\mathcal{L}} % Bounded operators
\newcommand{\cP}{\mathcal{P}} % Bounded operators
\newcommand{\cR}{\mathcal{R}} % Bounded operators
\newcommand{\cJ}{\mathcal{J}} % Bounded operators
\newcommand{\cC}{\mathcal{C}} % Bounded operators
\newcommand{\cQ}{\mathcal{Q}} % Bounded operators
\newcommand{\Sp}{\mathbf{S}} % Bounded operators
\newcommand{\BO}{\mathcal{B}} % Bounded operators
\newcommand{\DO}{\mathcal{D}} % Bounded operators
\newenvironment{smatrix}{\left(\begin{smallmatrix}}{\end{smallmatrix}\right)}
\renewcommand{\L}{\mathcal{L}} % graph Laplacian
\newcommand{\FO}{\mathcal{F}} % Finite rank operators
\newcommand{\KO}{\mathcal{K}} % compact operators
\newcommand{\landauo}[1]{
  \mathchoice
    {{\scriptstyle\mathcal{O}}}% \displaystyle
    {{\scriptstyle\mathcal{O}}}% \textstyle
    {{\scriptscriptstyle\mathcal{O}}}% \scriptstyle
    {\scalebox{.7}{$\scriptscriptstyle\mathcal{O}$}}%\scriptscriptstyle
  (#1)}
\newcommand{\stO}[1]{\mathcal{O}_\prec\left(#1\right)} 
\newcommand*{\defeq}{\mathrel{\vcenter{\baselineskip0.5ex \lineskiplimit0pt\hbox{\scriptsize.}\hbox{\scriptsize.}}}=}
\newcommand*{\defqe}{=\mathrel{\vcenter{\baselineskip0.5ex \lineskiplimit0pt\hbox{\scriptsize.}\hbox{\scriptsize.}}}}                     
\newcommand{\norms}[2][0]{%
  \ifcase#1\relax
    \lVert #2\rVert\or         % 0
    \big\lVert #2\big\rVert\or   % 1
    \Big\lVert #2\Big\rVert\or   % 2
    \bigg\lVert #2\bigg\rVert\or  % 3
    \Bigg\lVert #2\Bigg\rVert\or     % 4
    \left\lVert #2\right\rVert
  \fi
} 
\makeatletter
\def\norm{\@ifnextchar[{\@normwith}{\@normwithout}}
\def\@normwith[#1]#2{\norms[#1]{#2}}
\def\@normwithout#1{\norms[5]{#1}}
\makeatother
\newcommand{\tnorms}[2][0]{%
  \ifcase#1\relax
    \lvert\kern-0.25ex\lvert\kern-0.25ex\lvert #2 \rvert\kern-0.25ex\rvert\kern-0.25ex\rvert\or % 0
    \big\lvert\kern-0.25ex\big\lvert\kern-0.25ex\big\lvert #2 \big\rvert\kern-0.25ex\big\rvert\kern-0.25ex\big\rvert\or   % 1
    \Big\lvert\kern-0.25ex\Big\lvert\kern-0.25ex\Big\lvert #2 \Big\rvert\kern-0.25ex\Big\rvert\kern-0.25ex\Big\rvert\or   % 1
    \bigg\lvert\kern-0.25ex\bigg\lvert\kern-0.25ex\bigg\lvert #2 \bigg\rvert\kern-0.25ex\bigg\rvert\kern-0.25ex\bigg\rvert\or   % 1
    \Bigg\lvert\kern-0.25ex\Bigg\lvert\kern-0.25ex\Bigg\lvert #2 \Bigg\rvert\kern-0.25ex\Bigg\rvert\kern-0.25ex\Bigg\rvert\or   % 1
    \left\lvert\kern-0.25ex\left\lvert\kern-0.25ex\left\lvert #2 \right\rvert\kern-0.25ex\right\rvert\kern-0.25ex\right\rvert
  \fi
} 
\makeatletter
\def\tnorm{\@ifnextchar[{\@tnormwith}{\@tnormwithout}}
\def\@tnormwith[#1]#2{\tnorms[#1]{#2}}
\def\@tnormwithout#1{\tnorms[5]{#1}}
\makeatother
\newcommand{\abss}[2][0]{%
  \ifcase#1\relax
    \lvert #2\rvert\or         % 0
    \big\lvert #2\big\rvert\or   % 1
    \Big\lvert #2\Big\rvert\or   % 2
    \bigg\lvert #2\bigg\rvert\or  % 3
    \Bigg\lvert #2\Bigg\rvert\or     % 4
    \left\lvert #2\right\rvert
  \fi
} 
\makeatletter
\def\abs{\@ifnextchar[{\@abswith}{\@abswithout}}
\def\@abswith[#1]#2{\abss[#1]{#2}}
\def\@abswithout#1{\abss[5]{#1}}
\makeatother
\newcommand{\landauOs}[2][0]{%
  \ifcase#1\relax
    \mathcal{O}(#2)\or         % 0
    \mathcal{O}\big(#2\big)\or         % 1
    \mathcal{O}\Big(#2\Big)\or         % 2
    \mathcal{O}\bigg(#2\bigg)\or  % 3
    \mathcal{O}\Bigg(#2\Bigg)\or     % 4
    \mathcal{O}\left(#2\right)
  \fi
} 
\makeatletter
\def\landauO{\@ifnextchar[{\@landauOwith}{\@landauOwithout}}
\def\@landauOwith[#1]#2{\landauOs[#1]{#2}}
\def\@landauOwithout#1{\landauOs[5]{#1}}
\makeatother
\providecommand{\maxnorm}[1]{\left\lVert#1\right\lVert_{\text{max}}} %norm
\providecommand{\braket}[1]{\left\langle#1\right\rangle} %absolute value
\providecommand{\Cov}[1]{\mathbf{Cov}(#1)} %Cov
\providecommand{\CovBig}[1]{\mathbf{Cov}\Big(#1\Big)} %Cov
\providecommand{\Covbig}[1]{\mathbf{Cov}\big(#1\big)} %Cov
\providecommand{\floor}[1]{\lfloor#1\rfloor} %absolute value
\renewcommand{\implies}{\Rightarrow}
\DeclareMathOperator{\esssup}{ess~sup}
\DeclareMathOperator{\argmin}{arg~min}
\DeclareMathOperator{\argmax}{arg~max}

\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\vdeg}{vdeg}
\DeclareMathOperator{\VE}{VE}
\DeclareMathOperator{\GE}{GE}
\DeclareMathOperator{\WeE}{WE}
\DeclareMathOperator{\WE}{\GE_{\text{W}}}
\DeclareMathOperator{\IE}{IE}
\newcommand{\Nexp}{n}
\DeclareMathOperator{\Ed}{E}
\DeclareMathOperator{\arccot}{arccot}
\DeclareMathOperator{\Ran}{Ran}
\DeclareMathOperator{\dlim}{d-lim}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\Val}{Val}
\DeclareMathOperator{\WEst}{W-Est}
\DeclareMathOperator{\cco}{cc}
\DeclareMathOperator{\SVal}{SVal}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\interior}{int}
\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\maxroot}{maxroot}
\DeclareMathOperator{\arctanh}{arctanh}
\DeclareMathOperator{\E}{\mathbf{E}}
\DeclareMathOperator{\Var}{\mathbf{Var}}
\renewcommand{\P}{\mathbf{P}}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\wlim}{w-lim}
\DeclareMathOperator{\linspan}{span}
\DeclareMathOperator{\graph}{Gr} %Graph of a map f: X \to Y in X\times Y
\DeclareMathOperator{\dist}{dist} %Graph of a map f: X \to Y in X\times Y
\newcommand{\ba}{{\mathbf a}}
\newcommand\restr[2]{{% we make the whole thing an ordinary symbol
  \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  #1 % the function
  \vphantom{\big|} % pretend it's a little taller at normal size
  \right|_{#2} % this is the delimiter
  }}
\makeatletter
\providecommand*{\diff}%
        {\@ifnextchar^{\DIfF}{\DIfF^{}}}
\def\DIfF^#1{%
        \mathop{\mathrm{\mathstrut d}}%
                \nolimits^{#1}\gobblespace
}
\def\gobblespace{%
        \futurelet\diffarg\opspace}
\def\opspace{\let\DiffSpace\! \ifx\diffarg(\let\DiffSpace\relax\else\ifx\diffarg\let\DiffSpace\relax\else\ifx\diffarg\{\let\DiffSpace\relax\fi\fi\fi\DiffSpace}  
\newcommand{\cor}{\color{red}}
\newcommand{\cred}[1]{{\color{red} #1}}
\newcommand{\cblue}[1]{{\color{blue} #1}}
\newcommand{\cob}{\color{blue}}
\newcommand{\nc}{\normalcolor}
\newcommand{\ord}{\mathcal{O}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\scalar}[2]{\langle{#1} \mspace{2mu}, {#2}\rangle}
\newcommand{\vr}{\mathbf r}
\newcommand{\bels}[2] {
        \begin{equation} \label{#1} \begin{split} 
                #2 
        \end{split} \end{equation}
        }
\newcommand{\bes}[1]{
        \begin{equation*}  \begin{split} 
                #1 
        \end{split} \end{equation*}
        }
\newcommand{\bea}[1]{
  \begin{align*}
    #1
  \end{align*}
  }
\newcommand{\mtwo}[2]
{
\left(
\begin{array}{cc}
#1 
\\
#2
\end{array}
\right)
}
\renewcommand{\val}[1]{\Val\left(#1\right)}


%\newcommand{\ii}{\mathrm{i}} %\newcommand{\mi}{\mathrm{i}}
\renewcommand{\i}{\mathrm{i}} %imaginary part of a complex number
%\newcommand{\abs}[1]{\lvert #1 \rvert}

%norm
%\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\normtwo}[1]{\lVert #1 \rVert_{\mathrm{hs}}}
\newcommand{\normsp}[1]{\lVert #1 \rVert_{\mathrm{sp}}}
\newcommand{\normtwoinf}[1]{\lVert #1 \rVert_{\mathrm{hs}\to\norm{\cdot}}}


%average
\newcommand{\avg}[1]{\langle #1 \rangle}

%scalar product with angle brackets
\newcommand{\scalarbb}[2]{\bigg\langle{#1} \,\mspace{2mu},\, {#2}\bigg\rangle}
\DeclareMathOperator*{\sign}{sign}						%Signum
\DeclareMathOperator*{\spec}{Spec}						%Spectrum


\newcommand{\genarg} {{\,\cdot\,}}  % general argument: f(\genarg) produces dot with little space around it


%\renewcommand{\Im}{\mathrm{Im}\,} %imaginary part of a complex number
%\renewcommand{\Re}{\mathrm{Re}\,} %real part of a complex number

\newcommand{\di}{\mathrm{d}} % differential
\newcommand{\eps}{\varepsilon} % "correct" epsilon
%\newcommand*{\defeq}{\mathrel{\vcenter{\baselineskip0.5ex \lineskiplimit0pt\hbox{\scriptsize.}\hbox{\scriptsize.}}}=}
%\newcommand*{\defqe}{=\mathrel{\vcenter{\baselineskip0.5ex \lineskiplimit0pt\hbox{\scriptsize.}\hbox{\scriptsize.}}}}                     

\newcommand{\pt}{\partial}



\newcommand{\Hb}{\mathbb H}




\newcommand{\id}{I}
\newcommand{\Id}{\mathrm{Id}}
\newcommand{\charfunc}{\ensuremath{\mathbf{1}}} %Characteristic function

%\newcommand{\cF}{\mathcal{F}}
\newcommand{\cV}{\mathcal{V}}

\renewcommand{\SS}{\mathcal{S}}
\newcommand{\cA}{\mathcal{A}} %
%\newcommand{\cP}{\mathcal{P}} %
\newcommand{\cK}{\mathcal{K}} % 
%\newcommand{\cC}{\mathcal{C}} % 
%\newcommand{\cE}{\mathcal{E}} % 
%\newcommand{\cQ}{\mathcal{Q}} %
%\newcommand{\BO}{\mathcal{B}} % 
\newcommand{\TO}{\mathcal{T}} % 
%\newcommand{\DO}{\mathcal{D}} % 



\newcommand{\dens}{\varrho} 
\newcommand{\Dbdd}{\mathbb{D}^{\omega_*}}
\newcommand{\Dtheta}{\mathbb{D}^{\omega_*/2}}

